How Can Haptic Feedback Assist People with Blind and Low Vision (BLV): A Systematic Literature Review

People who are blind or have low vision (BLV) encounter numerous challenges in their daily lives and work. To support them, various haptic assistive tools have been developed. Despite these advancements, the effective utilization of these tools -- including the optimal haptic feedback and on-body stimulation positions for different tasks along with their limitations -- remains poorly understood. Recognizing these gaps, we conducted a systematic literature review spanning two decades (2004-2024) to evaluate the development of haptic assistive tools within the HCI community. Our findings reveal that these tools are primarily used for understanding graphical information, providing guidance and navigation, and facilitating education and training, among other life and work tasks. We identified three main limitations: hardware limitations, functionality limitations, and UX and evaluation methods limitations. Based on these insights, we discuss potential research avenues and offer suggestions for enhancing the effectiveness of future haptic assistive technologies.

==> source/copy_of_findings.tex <==
\section{Findings}
In this section, we first report how various haptic assistive tools (Section \ref{Haptic Assistive Tools for Various Tasks}), haptic feedback (Section \ref{Haptic Feedback for Various Tasks}), and on-body stimulation positions (Section \ref{Stimulation Position for Tasks}) can assist BLV people in different tasks. 
For each task type, feedback method, and stimulation position, we discuss associated challenges and potential opportunities. 
Following this overview, we offer a detailed analysis of the limitations of existing haptic tools, focusing on three perspectives: 1) Hardware limitations (Section \ref{Hardware limitations}) including environmental effects, conspicuousness, and form factor; 
2) Functionality limitations (Section \ref{Functionality limitations}) including control over information display, information resolution, and presentation modality;
and 3) UX and evaluation method limitations (Section \ref{UX and evaluation method limitations}), including user diversity, customization, user study design, and user trust.


% Then, we report the limitations of current haptic assistive tools. 

\subsection{Haptic Assistive Tools for Various Tasks} \label{Haptic Assistive Tools for Various Tasks}
Based on the task that each haptic assistive tool was designed to support, we summarized them into four main types and tallied the number of papers that apply to each task. They include 1) graphical information understanding (58/132), 2) guidance/navigation (26/132), 3) education/training (20/132), and 4) other life and work tasks (28/132). We classified the haptic assistive tools for each task based on their form factor, which refers to their size, shape, and physical specifications. The form factors include common assistive tools (e.g., tactile graphics/maps, refreshable braille display/pin arrays) and other haptic devices that may not be frequently used as assistive tools (e.g., haptic mice, haptic gloves, and haptic bands). The classification of papers is shown in Table \ref{table:type_of_haptic_assistive_tool}, while the Sankey diagram (Figure \ref{fig:task_haptic_assistive_tools}) illustrates the distribution of haptic assistive tools that assist various BLV tasks.

\begin{table}[htbh!]
\caption{Type of Haptic Assistive Tool}
\centering 
\small
\begin{tabular}{p{3cm}p{2.5cm}p{2.5cm}p{2.5cm}p{2.5cm}}

\hline
\textbf{Type of Haptic Assistive Tool} & \textbf{Graphical information understanding} & \textbf{Guidance/navigation} & \textbf{Education/training} & \textbf{Other life and work tasks}\\\hline
tactile graphics/maps & \cite{swaminathan2016linespace,li2019editing,yang2020tactile,hofmann2022maptimizer,holloway20223D,Nagassa20233D,baker2014tactile,lucentmaps2016gotzelmann,reichinger2016gesture,suzuki2017fluxmarker,baker2014tactile,visually2018gotzelmann,reichinger2018pictures,gupta2019evaluating,zeinullin2022tactile,kim2015toward,braier2014haptic,mcGookin2010clutching,wang2009instant,ducasse2016tangible,roberts2005haptic,mascle2022tactile} & /  & \cite{albouys2018towards,melfi2020understanding,fusco2015tactile,holloway20193d,sargsyan20233D}  & \cite{das2023simphony,bornschein2015collaborative,shi2020molder,pandey2020explore} \\\hline
refreshable braille displays/pin arrays & \cite{prescher2017consistency,besse2018understanding,prescher2010tactile,rao20202across,Deschamps2012interpersonal} & / & \cite{petit2008refreshable,saikot2022refreshable,melfi2022audio} & \cite{bornschein2018comparing,Jung2021ThroughHand,siu2019shapecad,Morash2018evaluating,russomanno2015refreshing,Siu2019Advancing,Cassidy2013haptic,Pantera2021lotusbraille} \\\hline
tablet/smartphone integrated haptic actuators & \cite{palani2017principles,chu2022comparative} & / & \cite{Toennies2011toward} & \cite{Rantala2009methods} \\\hline
haptic mice & \cite{brayda2015the,kim2011handscope,levesque2012adaptive,pietrzak2009creating} & / & \cite{brayda2013predicting} & \cite{Headley2011roughness,Strachan2013vipong} \\\hline
haptic gloves & \cite{soviak2016tactile,quek2013enabling,chase2020pantoguide} & / & \cite{oliveira2012the} & / \\\hline
haptic sliders & \cite{fan2022slide,gay2021f2t} & / & / & \cite{Tanaka2016haptic}      \\\hline
robot/drone haptic devices  & \cite{guinness2019robo,ducasse2018botmap} & \cite{huppert2021guidecopter,guerreiro2019cabot,kayukawa2020guiding,rahman2023take,moon2019prediction} & \cite{guinness2019robo} & / \\\hline
haptic bands & / & \cite{hong2017evaluating,erp2020tactile,Kaul2021around,hirano2019synchronized,cosgun2014evaluation,lee2023novel,barontini2021integrating,flores2015vibrotactile,xu2020virtual,ogrinc2018sensory} & / & \cite{sucu2014the,Stearns2016evaluating,Allman2009rock,kayhan2022a}    \\\hline
3D models & \cite{shi2016tickers,reinders2020hey,brule2021beyond,holloway2023tacticons,shi2017designing,kane2013touchplates,shi2019designing} & / & \cite{holloway2018accessible,davis2020tangible,chang2021accessiblecircuits} & \cite{Guo2017facade,baldwin2017the,lee2023tacnote}    \\\hline
white canes & / & \cite{siu2020virtual,swaminathan2021from,nasser2020thermalcane,zhao2018enabling,tanabe2021identification,wang2012halo,kim2015identification} & / & /   \\\hline
robotic-arm haptic devices & \cite{abu_doush2009making,abu2010multimodal,moll2013haptic,de_felice2007haptic,sallnas2007group,schloerb2010blindaid,park2015telerobotic} & / & \cite{zhang2017multimodal,espinosa2021virtual,crossan2008multimodal,plimmer2011signing,murphy2015haptics} & \cite{lieb2020haptic,Plimmer2008multimodal,Park2013real}   \\\hline
other handheld haptic devices & \cite{yatani2012spacesense,sharmin2005first} & \cite{liu2021tactile,amemiya2009haptic,amemiya2010orienting,spiers2017design} & \cite{sanchez2010usability} & \cite{Morelli2010vi}   \\\hline
electrotactile devices & \cite{jiang2024designing,yoo2022perception} & / & / & / \\\hline

\end{tabular}
\label{table:type_of_haptic_assistive_tool} 
% \description{Table 1 describes}
\end{table}

\begin{figure} [tbh!]
    \centering
    \includegraphics[scale=0.38]{figure/task_haptic_assistive_tools.jpg}
     \caption{Examples of haptic assistive tools designed for the four main types of tasks. The connections show which haptic tools assist the specific BLV tasks.}
     \Description{This figure illustrates the examples of 13 haptic assistive tools designed for the four main types of tasks. The numbers after each haptic assistive tool is the number of paper utilized the device}
    \label{fig:task_haptic_assistive_tools}
\end{figure}

\subsubsection{Haptic assistive tools for graphical information understanding}
\textit{Graphical information understanding} involves haptic assistive tools that support BLV people with comprehending the overview and details of any figure, chart, or map \cite{jiang2023understanding}. \textbf{Tactile graphics/maps} are the most common assistive tools for this purpose (22/58), followed by \textbf{3D models} (7/58) and \textbf{robotic-arm haptic devices} (7/58). 
\rv{The \textbf{robotic-arm haptic devices} utilize a robotic arm, such as Phantom $^\circledR$, to guide the BLV users during the learning process.
Its detailed applications for \textit{ducation/training} will be described in section \ref{Robotic_arm}.}

\textbf{Tactile graphics/maps} are the images that use raised dots, lines, and surfaces to convey graphical information \cite{tg}. 
The design considerations for different types of graphical information varied. 
In general, researchers focused on factors such as heights, widths, dashed patterns, and shapes of raised lines, dots, and surfaces to assist the three elemental tasks in graphical information understanding, including \textbf{map information understanding}, \textbf{chart information understanding}, and \textbf{figure information understanding}.

For \textbf{map information understanding}, researchers first determined which geographic features to include---such as roads, buildings, and other facilities \cite{hofmann2022maptimizer,Nagassa20233D,gupta2019evaluating}. 
They then decided how to represent these selected features. 
Some used raised lines to indicate roads, varying the width and dashed patterns to represent different road types, from footpaths to highways \cite{hofmann2022maptimizer}. 
Others employed raised spaces and raised dots of various shapes (e.g., triangles, squares) to convey textures representing different map areas \cite{hofmann2022maptimizer,holloway20223D,gupta2019evaluating}. 
Additionally, some researchers utilized movable 3D-printed icons to denote specific landmarks, such as restrooms or shops \cite{Nagassa20233D}.

\textbf{Chart information understanding} followed a similar approach, with the primary distinction being that researchers focused on which chart features to include rather than geographic features. 
This included methods to assist BLV users in distinguishing various bars, dots, lines, and slices \cite{braier2014haptic,baker2014tactile}.

For \textbf{figure information understanding}, researchers typically began by separating figures into various areas and layers based on their structures. 
For example, they separated the elephant's figure into its leg, body, ear, head, and teeth according to its taxonomy structure \cite{kim2015toward,gupta2019evaluating,reichinger2018pictures}. 
These different areas were generally displayed with height variations that reflected their real-world perspectives \cite{kim2015toward,gupta2019evaluating}. 
In contrast to map information, figure information was usually represented similarly to the original visualized figure \cite{reichinger2018pictures}. 
Additionally, while map information often used a single tactile graphic to represent the entire map, figure information sometimes employed multiple tactile graphics to convey different elements.

The design differences between maps and figures were informed by the nature of the information being conveyed to BLV users.
Map information design focused more on providing an overview, often omitting detailed elements or relying on audio feedback for additional details. 
\rv{This is because tactile graphics provide lower spatial acuity compared to visual perception because getting information by touch is more “sequential” than vision.
In comparison, audio lacks spatial constraints and can convey information temporally \cite{}}
In comparison, the specifics were crucial for figure information, necessitating designs that closely resembled the original figures.
An example of maps is a 3D Building Plan developed by Nagassa et al. to show multi-story buildings' indoor structures. They found that BLV users preferred the overlapped presentations, a movable stack of each floor's tactile map, shown in Figure \ref{fig:tactile_graphics} c). The overlapped presentations enabled more effective building of cross-floor spatial overview \cite{Nagassa20233D}. Swaminathan et al. leveraged 3D printers to create a refreshable tactile display system by printing the raised lines of filament in real-time, shown in Figure \ref{fig:tactile_graphics} a). They found that their design is more expressive compared to the traditional refreshable braille displays which present graphics with dots \cite{swaminathan2016linespace}. 

\begin{figure} [tbh!]
    \centering
    \includegraphics[scale = 0.8]{figure/tactile_graphics.jpg}
     \caption{Examples of tactile graphics/maps: a) Linespace: a refreshable tactile graphic system based on 3D printers \cite{swaminathan2016linespace}; b) a mobile audio-tactile system for learning graphics at schools \cite{melfi2020understanding}; c) 3D Building Plans: a 3D-printed multi-story building tactile map for O\& M education. The figure shows one of the three designs in which the users can slide away each layer of the tactile map \cite{Nagassa20233D}.}
    \Description{This figure illustrates the examples of tactile graphics/maps, each figure includes three subfigures. Each subfigure shows one prototype.}

    \label{fig:tactile_graphics}
\end{figure}


\textbf{3D models} are the second most used haptic assistive tools to assist in graphical information understanding, including either wooden or 3D-printed models that convey spatial information \cite{holloway2023tacticons}.

When designing these models, researchers focused on ensuring they could be easily distinguished by users. 
Some created 3D models based on real-world objects and referenced familiar visual icons, such as flowers, signs, and buildings, which are easily recognizable and memorable \cite{holloway2023tacticons,shi2017designing,shi2019designing}. 
They transformed these 2D icons into 3D models by following their real-world outlines \cite{holloway2023tacticons}. 
Additionally, some researchers incorporated removable components to allow users to explore the details. 
These models closely resembled actual structures and were often utilized in formal contexts, such as science popularization and education/training \cite{reinders2020hey}. 
Recently, 3D models have commonly been integrated with audio labels, supporting users' understanding of various parts of the models, such as continents on a globe or components within a cell \cite{shi2019designing,shi2016tickers}.

For example, Holloway et al. developed a series of 3D-printed icons to assist BLV people in recognizing landmarks on maps as efficiently as sighted people, which is shown in Figure \ref{fig:3D_models} a). They found that BLV participants can learn their 3D-printed icons easily and recognize them instantly. \cite{holloway2023tacticons}. Davis et al. presented a multimodal device that allows BLV users to understand circuit diagrams by interacting with 3D-printed circuit tangible models, which is shown in Figure \ref{fig:3D_models} b). They found that BLV users can better understand the geometric, spatial, and structural circuit information using their device \cite{davis2020tangible}.

Additionally, electrotactile devices, illustrated in Figure \ref{fig:electrotactile_devices}, utilize electric current applied directly to the skin or through a thin insulating layer with conductive material to generate tactile sensations \cite{yoo2022perception,jiang2024designing}. 
Researchers have focused on various features of modulated electrical signals, including voltage, current, frequency, stimulation duration, and intervals \cite{lin2022super}.



\begin{figure} [tbh!]
    \centering
    \includegraphics[scale = 0.8]{figure/3D_models.jpg}
     \caption{Examples of 3D models: a) TactIcons: 3D printed icons that can substitute visual icons for street and park tactile maps \cite{holloway2023tacticons}; b) TangibleCircuits: a haptic and audio feedback device based on 3D models that allow BLV users to understand circuit diagrams \cite{davis2020tangible}; c) Tangible Desktop: 3D-printed icons for multimodal interaction of computers. Each icon has an RFID tag embedded inside and a tactilely distinct rubber crown \cite{baldwin2017the}.}
     \Description{This figure illustrates the examples of 3D models, each figure includes three subfigures. Each subfigure shows one prototype.}
    \label{fig:3D_models}
\end{figure}


\begin{figure} [tbh!]
    \centering
    \includegraphics[scale = 0.8]{figure/electrotactile_devices.jpg}
     \caption{Examples of Electrotactile Devices: a) an assistive tool based on unobtrusive modulated electrotactile feedback on fingertip Edge for charts comprehension \cite{jiang2024designing}; b) An electrostatic skin-stretch display for graphics exploration  \cite{yoo2022perception}.}
     \Description{This figure illustrates the examples of electrotactile devices with two subfigures. Each subfigure shows one prototype.}
    \label{fig:electrotactile_devices}
\end{figure}

\subsubsection{Challenges in graphical information understanding}
Based on our literature survey, we synthesized the main challenges that exist in \textit{graphical information understanding}, which include \textbf{low comprehension efficiency of the overview}, \textbf{difficulty with detail gathering}, and \textbf{high short-term memory load} \cite{fan2023accessibility, baldwin2017the}. 
\rv{The challenges of \textbf{low comprehension efficiency of the overview} and \textbf{difficulty with detail gathering} arise because BLV individuals must rely on audio descriptions of alternative text or explore tactile graphics with their fingers to understand details at each location. 
This step-by-step process to construct an overview is more time-consuming than the experience of sighted individuals \cite{jiang2023understanding}. 
Moreover, building an overview requires BLV people to retain details quickly and precisely, which imposes a \textbf{high short-term memory load} \cite{baldwin2017the}.
}

\textbf{Low comprehension efficiency of the overview} and \textbf{difficulty with detail gathering}: 
Haptic devices often support users in grasping both the overview and intricate details of figures or maps. 
Initially, these devices guide users through the overall structure to establish a foundational understanding of the charts or figures. 
Subsequently, they facilitate free exploration to deepen comprehension. For instance, Abu-doush's robotic-arm haptic devices offer guided and exploratory modalities.
The guided mode directs users' fingers along predefined trajectories to comprehend trends in line charts, while the exploratory mode enables users to explore individual bars or slices in bar or pie charts \cite{abu2010multimodal}.

\textbf{High short-term memory load}: 
High short-term memory load presents another obstacle with graphical information understanding. 
Previous studies identified note-taking as a strategy to alleviate this burden \cite{lee2023tacnote, pandey2020explore}.
However, for BLV individuals, conventional note-taking methods can be challenging due to the difficulty in retrieving data and the inconvenience of switching between note-taking applications \cite{jiang2023understanding}.
To address this issue, Lee et al. investigated the use of a 3D printing pen to facilitate note-taking by creating tangible 3D models.
Through tactile exploration, BLV users could specify the locations, ordering, and hierarchy relationships of notes, effectively reducing their memory load \cite{lee2023tacnote}.
Despite the potential of haptic devices to address various challenges, most focus solely on aiding comprehension of overviews and details. 
Few explore methods to mitigate short-term memory load, highlighting a promising area for further research.

\subsubsection{Haptic assistive tools for guidance/navigation}
\textit{Guidance/Navigation} involves haptic assistive tools that support BLV people with finding directions or specific objects in indoor and outdoor scenarios \cite{csapo2015survey}. \textbf{Haptic bands} (10/26) and \textbf{white canes} (8/26) are the most used haptic assistive tools. 

The \textbf{haptic bands} are bands that are equipped with haptic actuators (e.g., vibrators) and are bound to the user's arm, wrist, or waist. 
The design of haptic bands typically focused on accurately conveying guidance cues and mapping them to real-world directions. 
Researchers first considered the arrangement of actuators around the bands, including their number, type, and density \cite{hong2017evaluating}. 
Normally, the higher number of vibrators could ensure denser arrangments, and thus convey more precise guidance cues \cite{hong2017evaluating}.
They then determined the vibration patterns for guidance and notification cues, which included both single and sequential vibrations \cite{hong2017evaluating,xu2020virtual}. 
Single vibrations activated the vibrator closest to the target direction \cite{flores2015vibrotactile}, while sequential vibrations involved more complex patterns, with the direction indicated from the vibration start point to the endpoint \cite{hong2017evaluating, Kaul2021around, ogrinc2018sensory,lee2023novel}. 
Some designs incorporated multiple vibrations, where rotational vibrations around the arms or wrists signified turning directions—clockwise for right turns and counterclockwise for left turns \cite{ogrinc2018sensory}.

Additionally, vibration durations, intervals, and overlaps were considered to convey notifications. 
The combination of different stimulation durations and pauses can indicate various states, such as attention, walking, stopping, and barriers ahead of the users \cite{lee2023novel}.

For example, Lee et al. presented a wrist-worn vibrotactile device to provide directional, spatial, and status cues to assist BLV people's independent walking and wayfinding, shown in Figure \ref{fig:haptic_bands} c). They found that their vibrotactile information was quickly identified and it enabled BLV users to walk independently without any pre-learned knowledge about the route\cite{lee2023novel}. Barontini et al. developed a wearable system to assist BLV people in indoor navigation and obstacle avoidance, shown in Figure \ref{fig:haptic_bands} b). They found that their device could support indoor navigation and allowed BLV people to travel independently \cite{barontini2021integrating}. 

\begin{figure} [tbh!]
    \centering
    \includegraphics[scale = 0.8]{figure/haptic_bands.jpg}
     \caption{Examples of haptic bands: a) A vibrotactile band worn on the hand to assist BLV drivers through vibration cues \cite{sucu2014the}; b) A haptic band based on vibration worn on the BLV users' arms to provide guidance cues \cite{barontini2021integrating}; c) A haptic band worn on the arm to assist BLV users in independent travel through eight vibrators \cite{lee2023novel}.}
     \Description{This figure illustrates the examples of haptic bands, each figure includes three subfigures. Each subfigure shows one prototype.}
    \label{fig:haptic_bands}
\end{figure}

\textbf{White canes} are the second most used haptic assistive tools to assist in guidance/navigation. White canes are sticks between 100 to 150 centimeters in length that help BLV people detect obstacles on the road, which may be equipped with either thermal modules \cite{nasser2020thermalcane} or vibrators \cite{siu2020virtual}.

The design of white canes focused on effectively conveying directional cues and notifying users of barriers, including their direction, distance, and height \cite{wang2012halo,kim2015identification,siu2020virtual}. 
Notification cues could be delivered through vibrators and mechanical brakes \cite{siu2020virtual}. 
Some researchers utilized brakes to provide resistance and vibrators to simulate various textures encountered on the ground, such as carpets, tactile pavements, or walls \cite{siu2020virtual,zhao2018enabling,tanabe2021identification}. 
Obstacles were typically indicated by single vibrations to convey their locations (using different positions on the white cane) and heights (through varying vibration frequencies) \cite{wang2012halo,kim2015identification}.

Additionally, some studies explored how to convey directional cues using white canes, with design considerations similar to those of haptic bands, including the number, type, and density of actuators. 
The key difference was that white canes were held by users rather than worn on their arms or wrists, meaning that the holding posture affected how guidance cues were mapped, which was an important consideration in their design \cite{nasser2020thermalcane}.


For example, Nasser et al. developed Thermalcane, a white cane that can offer thermotactile directional cues for BVI users, shown in Figure \ref{fig:white_canes} b). They found that the thermal feedback yielded significantly higher accuracy than the vibrotactile feedback used with white cane \cite{nasser2020thermalcane}. Siu et al. developed a multimodal cane controller that provides texture simulation and spatialized audio, shown in Figure \ref{fig:white_canes} a). They found that their device allows BLV people to navigate in large virtual environments with complex architecture without vision \cite{siu2020virtual}. 



\begin{figure} [tbh!]
    \centering
    \includegraphics[scale = 0.8]{figure/white_canes.jpg}
     \caption{Examples of white canes: a) A white cane integrated with vibrators to guide BLV users in VR environment \cite{siu2020virtual}; b) A white cane integrated with Peltiers that can guide BLV users via thermal feedback \cite{nasser2020thermalcane}; c) HALO: A white cane integrated with vibrators to assist BLV people in recognizing low-hanging obstacles such as tree branches and open cabinet doors \cite{wang2012halo}.}
     \Description{This figure illustrates the examples of white canes, each figure includes three subfigures. Each subfigure shows one prototype.}
    \label{fig:white_canes}
\end{figure}

\subsubsection{Challenges in guidance/navigation}
The main challenges of \textit{guidance/navigation} based on our literature review include \textbf{disorientation with directions}, \textbf{difficulty with avoiding obstacles and crowds}, \textbf{risk of falling}, and \textbf{risks associated with intersection crossings} \cite{riazi2016outdoor}. 
\rv{
The challenge of \textbf{disorientation with directions} arises because BLV individuals often struggle to identify landmarks, making it difficult to understand their current location and decide on the next steps. 
Additionally, the lack of visual input complicates the recognition of approaching pedestrians, obstacles, and height differences between road surfaces. 
This, in turn, leads to challenges such as \textbf{difficulty avoiding obstacles and crowds}, an increased \textbf{risk of falling}, and heightened \textbf{risks associated with crossing intersections} \cite{riazi2016outdoor}.
}

\textbf{Disorientation with directions}: 
Certain haptic devices address the challenge of disorientation with directions via haptic cues. 
For instance, tactile graphics/maps, mid-air haptic devices, and haptic sliders offer tactile representations of maps, enabling BLV users to familiarize themselves with environments prior to actual navigation \cite{Nagassa20233D,fink2023autonomous,gay2021f2t}.

\textbf{Difficulty with avoiding obstacles and crowds}: 
Haptic notifications are provided by tools like haptic bands, white canes, handheld haptic devices, and robot/drone haptic devices, aiding users in navigation and obstacle avoidance  \cite{lee2023novel,barontini2021integrating,liu2021tactile,huppert2021guidecopter,nasser2020thermalcane,kayukawa2020guiding,guerreiro2019cabot}.
These devices offer real-time cues for independent travel, alerting users to obstacles or pedestrians along their path.

\textbf{Risk of falling}: 
The risk of falling is effectively addressed by white canes and robots, as they offer physical support between BLV users and the ground, substantially reducing the likelihood of falls \cite{nasser2020thermalcane,kayukawa2020guiding,guerreiro2019cabot}. 
Unlike haptic bands, handheld haptic devices, and drones, which are either worn or held by users, white canes and guiding robots can establish robust physical support, enhancing users' stability and safety during navigation \cite{lee2023novel,barontini2021integrating,liu2021tactile,huppert2021guidecopter}. 

\textbf{Risks associated with intersection crossings}: 
Our literature review did not identify any papers specifically addressing the challenge of \textit{risks associated with intersection crossings}. 
While previous studies have investigated auditory feedback to aid BLV individuals in street crossing, concerns about auditory distractions from surrounding noise have been raised \cite{borenstein1997guidecane,velazquez2010wearable}. 
Therefore, there is potential for future research to explore the use of haptic cues to assist BLV individuals in safely navigating intersections.
Developing haptic devices capable of providing guidance cues and preventing falls could greatly enhance the safety and independence of BLV individuals during street crossings.




\subsubsection{Haptic assistive tools for education/training}
% \textit{Education/Training} is how BLV people are assisted in STEM education, Orientation and Mobility (O\&M) training, and other skill learning. 
\textit{Education/Training} includes various disciplines such as STEM education, Orientation and Mobility (O\&M) training, and other skill learning. 
BLV people participate O\&M training to learn skills to travel safely and efficiently through their environment, such as wayfinding/orientation, street crossings, public transit, and use of GPS and electronic travel aids \cite{wiener2010foundations}. Papers on assistive tools for O\&M training study how the devices can be used to train users in a controlled environment with instructors, which is different from guidance/navigation tasks in which the users travel alone with the tools' assistance. \textbf{Tactile graphics/maps} (5/20) and \textbf{robotic-arm haptic devices} (5/20) are the most used haptic assistive tools for this task. 

For \textbf{tactile graphics/maps}, design considerations are similar to those for \textbf{graphical information understanding}. 
A key consideration is that researchers often designed tactile graphics/maps to be detachable or include movable 3D icons, allowing instructors to let BLV students explore them separately, which facilitates progressive teaching \cite{sargsyan20233D,holloway20193d}. 
Additionally, enabling teachers to easily modify audio descriptions for various locations and facilities on the tactile graphics/maps is another important design aspect. 
This flexibility allowed educators to guide students from basic recognition to a deeper understanding, transitioning from simply knowing names to comprehending the specific functions of different locations and facilities \cite{sargsyan20233D,fusco2015tactile,melfi2020understanding}.


For example, Melfi et al. introduced a mobile audio-tactile learning environment to facilitate BLV students' visual information learning, shown in Figure \ref{fig:tactile_graphics} b). They found that their device is suitable for educational environments because it allows faster exploration of tactile graphics and better memorization of information \cite{melfi2020understanding}. Sargsyan et al. developed 3D-printed tactile maps of a train station to teach the BLV people about complex spatial knowledge, part of  O\&M training. They found that complex spatial notions are better understood with their 3D maps compared to traditional 2D tactile maps \cite{sargsyan20233D}. 

\textbf{Robotic-arm haptic devices} are the second most used haptic assistive tools to assist in education/training. 
\label{Robotic_arm}
% The \textbf{robotic-arm haptic devices} utilize a robotic arm, such as Phantom $^\circledR$, to guide the BLV users during the learning process, including two elemental tasks: \textbf{2D structures learning} and \textbf{3D structures learning.}
\rv{The \textbf{robotic-arm haptic devices} were utilized for two elemental tasks: \textbf{2D structures learning} and \textbf{3D structures learning.}
}
Due to their high degree of freedom (DOF), the design of robotic-arm haptic devices emphasized encoding 2D and 3D information through the cursor's movement, force, and vibration. 

For \textbf{2D structures learning}, the robotic arm typically operated in an x-y plane, parallel to the ground, with movements indicating the outlines of figures or the trends of charts \cite{zhang2017multimodal,crossan2008multimodal,plimmer2011signing}. 
Applied forces, such as gravity acting vertically and viscosity opposing the user’s movement, helped notify users when they are on the correct trajectory along a figure's outline or a line chart \cite{zhang2017multimodal,abu2010multimodal}. 
This design rationale ensured that users perceive certain areas as more significant, encouraging them to continue moving along the designated lines or locations \cite{zhang2017multimodal,abu2010multimodal}. 
Additionally, vibrators installed on the cursor convey notification cues, indicating whether users are out of bounds or on a specific data point, thereby signaling when they are in a special location on the figure or chart \cite{abu2010multimodal}.

For \textbf{3D structures learning}, design considerations are similar to those of 2D figures, but the cursor moves within a 3D space. 
Researchers often employed forces to signal collisions with 3D objects and use vibrations to mark points of interest \cite{murphy2015haptics,espinosa2021virtual}.

In addition to facilitating independent learning, researchers also focused on increasing teacher involvement in the educational process. 
One design allows the robotic arm to follow the teacher’s movements in real-time, enabling students to mimic these movements instead of the pre-defined trajectories. 
This approach empowers teachers to instruct and correct students' mistakes immediately \cite{plimmer2011signing}.


% For example, Espinosa et al. explored how haptic feedback can support BLV students in learning math, particularly fundamental three-dimensional (3D) shapes, shown in Figure \ref{fig:robotic_arm_haptic_devices} b). They found that haptic virtual perception is a valid and effective assistive technology for the education of blind children \cite{espinosa2021virtual}. Zhang et al. developed a real-time multimodal image perception system with the user of robotic arms to assist BLV students'STEM course learning. They found that their device produced higher accuracy in recognizing images compared to conventional tactile images \cite{zhang2017multimodal}. 

\begin{figure} [tbh!]
    \centering
    \includegraphics[scale = 0.8]{figure/robotic_arm_haptic_devices.jpg}
     \caption{Examples of robotic-arm haptic devices: a) a multimodal robotic-arm haptic device that assists BLV people to build 3D models independently \cite{lieb2020haptic}; b) A robotic-arm haptic device that assists BLV people's education. The figure shows how it supports the BLV students in comprehending various shapes \cite{espinosa2021virtual}; c) A robot and robotic arm system to assist BLV people in telepresence \cite{Park2013real}.}
     \Description{This figure illustrates the examples of robotic-arm haptic devices, each figure includes three subfigures. Each subfigure shows one prototype.}
    \label{fig:robotic_arm_haptic_devices}
\end{figure}

\subsubsection{Challenges in education/training}
For \textit{education/training}, challenges include \textbf{difficulty following the blackboard and slice presentations}, \textbf{difficulty communicating with sighted classmates}, and \textbf{low efficiency in learning knowledge based on graphical information}. 
\rv{
The challenge of \textbf{difficulty following the blackboard and slice presentations} is induced when BLV people are unable to identify the specific location where the teacher is pointing—whether with a hand during face-to-face classes or with a cursor in online settings. 
Additionally, the lack of visual access contributes to \textbf{low efficiency in learning knowledge based on graphical information}, mirroring the challenges associated with \textit{graphical information understanding}. 
This divergence in learning processes, coupled with an inability to fully follow the teacher’s explanations, often leads to \textbf{difficulty following the blackboard and slice presentations}.
}

\textbf{Difficulty following the blackboard and slice presentations}: 
Haptic gloves have been utilized to address the challenge of difficulty following the blackboard and slice presentations. 
Oliveira et al. devised a system that tracked both the instructors' hand movements on the blackboard and the BLV students' hand movements on tactile graphics, which were proportionally scaled representations of the graphics displayed on the blackboard.  
Vibration feedback guided the students' hands to the corresponding positions on the tactile graphics based on where the instructors' hands pointed on the blackboard \cite{oliveira2012the}. 
However, the system's bulkiness and large size raise concerns about its impact on the learning experience of sighted classmates, potentially obstructing their view of the presentations. 
Hence, there is a need to address how BLV students can effectively follow instructors without impeding the learning of other students.

\textbf{Difficulty communicating with sighted classmates}: 
No paper in our literature review looked into how to support BLV students in effectively communicating their ideas and knowledge with sighted classmates.
Researchers have highlighted that the lack of communication of class content with classmates could potentially diminish students' learning efficiency \cite{you2021difference}. 
Although it is important for BLV students to effectively communicate with their sighted peers, they typically rely on haptic assistive tools, such as tactile graphics, to convey precise graphical information by indicating specific lines and areas \cite{d2021accessible}. 
Future research could focus on facilitating BLV students in creating their own tactile graphics more efficiently, which could enhance their ability to communicate with sighted classmates.

\textbf{Low efficiency in learning knowledge based on graphical information}:  
Tactile graphics/maps, refreshable braille displays, 3D models, and robotic-arm haptic assistive tools have emerged as effective solutions to address the challenge of low efficiency in learning knowledge based on graphical information \cite{albouys2018towards,holloway2018accessible,saikot2022refreshable,zhang2017multimodal,espinosa2021virtual}. 
These tools empower BLV students to explore figures, charts, and maps by utilizing finger movement and sensing height differences, enabling them to comprehend the spatial relationships within these graphical representations  \cite{albouys2018towards,holloway2018accessible,saikot2022refreshable}. Additionally, robotic-arm haptic assistive tools offer both guided navigation and free exploration, facilitating users in developing an overview through guidance and comprehending details through exploration \cite{zhang2017multimodal,espinosa2021virtual}. 
However, existing haptic assistive tools primarily target commonly used charts such as line charts, scatterplots, bar charts, and pie charts, with limited exploration of more complex chart types like radar charts, heat maps, and Sankey diagrams  \cite{fan2022slide,abu2010multimodal,chase2020pantoguide}. 
Hence, there is a \rv{short-term} opportunity for researchers to innovate and develop haptic devices capable of supporting BLV students in comprehending these less-studied chart formats.
\rv{In the long term, researchers could investigate more effective non-visual approaches for data sensemaking.
Based on these advancements, haptic devices leveraging the new methodologies could be developed to enhance data acquisition for BLV users.}


\subsubsection{Haptic assistive tools for other life and work tasks}
\textit{Other life and work tasks} consisted of the elemental tasks that BLV people conduct during their daily life and work, which less than five papers focused on. 

These elemental tasks include hand drawing/writing \cite{bornschein2018comparing,Plimmer2008multimodal,pandey2020explore}, braille reading \cite{Morash2018evaluating,russomanno2015refreshing,Rantala2009methods,Pantera2021lotusbraille}, gaming \cite{Jung2021ThroughHand,Allman2009rock,Morelli2010vi,Strachan2013vipong}, interacting with appliances \cite{Guo2017facade,baldwin2017the,Cassidy2013haptic}, using 3D modeling software \cite{siu2019shapecad,lieb2020haptic,Siu2019Advancing}, driving \cite{fink2023autonomous,sucu2014the}, designing assistive tools \cite{bornschein2015collaborative,shi2020molder}, presenting the roughness texture on tactile graphics \cite{Headley2011roughness}, weaving \cite{das2023simphony}, taking notes \cite{lee2023tacnote}, producing audio work \cite{Tanaka2016haptic}, and providing telepresence \cite{Park2013real}. 
\textbf{Refreshable braille displays/pin arrays} (8/28), \textbf{tactile graphics/maps} (4/28), and \textbf{haptic bands} (4/28) are the most used haptic assistive tools.

\begin{figure} [tbh!]
    \centering
    \includegraphics[scale = 0.8]{figure/mid_air_devices.jpg}
     \caption{Examples of mid-air devices: A mid-air haptic device to assist BLV drivers in comprehending street maps \cite{fink2023autonomous}.}
    \label{fig:mid_air_devices}
    \Description{This figure illustrates the examples of mid air devices, each figure includes three subfigures. Each subfigure shows one prototype.}
\end{figure}

\begin{figure} [tbh!]
    \centering
    \includegraphics[scale = 0.8]{figure/haptic_sliders.jpg}
     \caption{Examples of haptic sliders: a) Slide-Tone and Tilt-Tone: a system that assists BLV users in comprehending line charts. The figures showed the designs of the Slide-Tone device which conveys y-axis value in each x-axis value, and the Tilt-Tone device which conveys inclination in each x-axis value \cite{fan2022slide}; b) Haptic Wave: a haptic slider to assist BLV people in audio producing \cite{Tanaka2016haptic}; c) F2T: a haptic slider device that assists BLV people in understanding 2D maps \cite{gay2021f2t}.}
     \Description{This figure illustrates the examples of haptic sliders, each figure includes three subfigures. Each subfigure shows one prototype.}
    \label{fig:haptic_sliders}
\end{figure}

\textbf{Refreshable braille display/pin array} is an electro-mechanical device for displaying braille characters and figures by round-tipped pins and surfaces \cite{rbd}. For example, Siu et al. developed a 2.5D shape display that enables BLV designers to explore and modify existing models\cite{siu2019shapecad}. Jung et al. developed a device that enables BLV users to interact with multiple dynamic objects in real-time and thus play 2D games \cite{Jung2021ThroughHand}. 

For \textbf{tactile graphics/maps}, Das et al. presented an audio-tactile system that aims to support blind weavers in creating and perceiving patterns. They revealed how blind weavers used their devices to learn the process of pattern design and generate patterns with sighted instructors \cite{das2023simphony}. Lee et al. explored opportunities to enable object-centric note-taking using a 3D printing pen for interactive, personalized tactile annotations. Their device efficiently assisted BLV users in notetaking \cite{lee2023tacnote}. 

Additionally, researchers also presented other haptic assistive tools to support interacting with appliances via 3D models \cite{Guo2017facade,baldwin2017the}, driving via mid-air haptic devices \cite{fink2023autonomous} shown in Figure \ref{fig:mid_air_devices} a),  and haptic bands \cite{sucu2014the}, assisting audio production with haptic sliders shown in Figure \ref{fig:haptic_sliders} b) \cite{Tanaka2016haptic}, providing roughness on graphics with haptic mice\cite{Headley2011roughness} shown in Figure \ref{fig:haptic_mice} c), and providing telepresence via robotic-arm haptic devices \cite{Park2013real}.
Mid-air haptic devices could deliver unobtrusive haptic feedback directly to users' hands without requiring physical contact, enabling remote interactions. 
Although only one paper in our corpus explored the application of a mid-air assistive tool, its advantages---such as ease of use and remote interaction—suggest its potential for wider application in public assistive tools \cite{paneva2020haptiread}.


% The mid-air haptic devices could deliver unobtrusive haptic information directly to the user without touching any device, which allowed remote interactions.
% Though in our venue only one paper introduced the application of a mid-air assistive tool, its benefit of easy-to-operate and remote interaction may allow the application of public assistive tools.




\begin{figure} [tbh!]
    \centering
    \includegraphics[scale = 0.8]{figure/refreshable_braille_displays_pin_arrays.jpg}
     \caption{Examples of refreshable braille displays/pin arrays: a) A refreshable braille display that assists BLV people's drawing \cite{bornschein2018comparing}; b) ThroughHand: a pin array system that assists BLV people in playing 2D games \cite{Jung2021ThroughHand}; c) Audio-Tactile Reader (ATR): a multimodal refreshable braille display that assists in BLV people's STEM education \cite{melfi2022audio}.}
    \label{fig:refreshable_braille_displays_pin_arrays}
    \Description{This figure illustrates the examples of refreshable braille displays/pin arrays, each figure includes three subfigures. Each subfigure shows one prototype.}
\end{figure}

\begin{figure} [tbh!]
    \centering
    \includegraphics[scale = 0.8]{figure/haptic_mice.jpg}
     \caption{Examples of haptic mice: a) a haptic mouse that assists BLV people in comprehending 3D shapes for their O\& M education \cite{brayda2013predicting}; b) ViPong: a haptic mouse to assist BLV people in playing games \cite{Strachan2013vipong}; c) a haptic mouse that assists BLV people in understanding graphics with different details \cite{Park2013real}.}
     \Description{This figure illustrates the examples of haptic mice, each figure includes three subfigures. Each subfigure shows one prototype.}
    \label{fig:haptic_mice}
\end{figure}

\subsection{Underexplored Haptic Tools for Specific Tasks - Discussion for Haptic Assistive Tools for Various Tasks} \label{Haptic Assistive Tools for Understudied Application areas}
In our review of how haptic assistive devices are used for different tasks, we identified several areas with limited exploration in their applications. 
Specifically, we found no instances of haptic bands being employed to aid in understanding graphical information. 
For guidance and navigation purposes, only robot/drone haptic devices, haptic bands, white canes, and other handheld haptic devices were used. 
In the context of education and training, there was no use of haptic sliders and haptic bands. 
% Similarly, haptic gloves, robot or drone haptic devices, and white canes were not used for other life and work tasks.
These areas represent opportunities for further investigation, and we discuss potential avenues for future research in applying different haptic assistive tools for these tasks. 

\subsubsection{Underexplored haptic tools for graphical information understanding}
We found that haptic bands were not used to understand graphical information. 
% One possible explanation is that BLV people often use their fingers to interact with haptic displays.
This may be due to the nature of the task since perceiving detailed graphical elements requires precision, which is more typically conducted through direct and tactile finger-based interactions.
These interactions allow \rv{the BLV people} to perceive the variations in height across the graphs through devices like refreshable braille displays, pin arrays, and tactile graphics \cite{swaminathan2016linespace,Nagassa20233D,baker2014tactile}. 
Additionally, \rv{the BLV users} rely on haptic devices to guide their fingers along the contours of the graphs. 
Examples of such guiding devices include robot or drone haptic devices and robotic-arm haptic devices \cite{guinness2019robo,ducasse2018botmap,abu2010multimodal}.
In contrast, haptic bands are typically worn on the arm, wrist, and waist, and offer guidance information with a resolution of a few centimeters. 
As a result, they may be less effective at conveying graphical information, which requires more fine-grained resolution.
However, the key function of haptic devices for graphical information understanding involves providing details about the graphs' outlines and helping BLV people traverse and explore these graphs \cite{abu2010multimodal,fan2022slide,swaminathan2016linespace}.
Therefore, if the haptic band is small enough to be worn on the finger and convey guidance at a centimeter level, it may effectively guide the BLV users' fingers in exploring the graphs.

In addition, only two papers in our corpus explored the application of electrotactile devices for understanding graphical information.
However, their low cost, lightweight design, flexibility, and high guidance resolution suggest potential applications in graphical information understanding, as users could explore detailed graphics for a long time \cite{jiang2024designing}.

% In addition to haptic rings, no white canes have been used to assist graphical information understanding because users commonly hold white canes to detect obstacles on the road, which requires its length to be more than one meter, even longer than the graphs to be explored \cite{nasser2020thermalcane,siu2020virtual}.
% Therefore, white canes may be unsuitable to assist BLV users with graphical information understanding tasks.

\subsubsection{Underexplored haptic tools for guidance/navigation}
We found that only robot/drone haptic devices, haptic bands, white canes, and other handheld haptic devices were used for guidance/navigation. 
\rv{The refreshable braille displays/pin arrays, tablet/smartphone integrated haptic actuators, and haptic gloves can assist with guidance/navigation after further improvement. }
The potential reasons are that the haptic devices should be wearable and portable enough to be brought outdoors. 
Additionally, they should either be able to continuously guide the BLV users relative to the current direction and location \cite{huppert2021guidecopter,hong2017evaluating} (e.g., robot/drone haptic devices, haptic bands, etc), or should be able to detect obstacles and people passing by in real-time \cite{nasser2020thermalcane,swaminathan2021from} (e.g., white canes). 
However, tactile graphics/maps are usually non-refreshable and non-zoomable, which cannot fulfill the requirement of continuous guidance and real-time obstacle detection. 
Although prior work has developed refreshable and zoomable tactile graphics using a 3D printer to print the required detailed images in real time \cite{swaminathan2016linespace}, current 3D printers are not portable and thus the BLV users cannot wear or hold the device to guide them. 

In contrast, refreshable braille displays/pin arrays may provide continuous guidance cues by rendering the guidance information.
For example, when the BLV users hold the device, the pins could arise and fall to form an arrow in the display that always points to the correct directions. 
In addition, it can display surrounding maps to the BLV users that include important information, such as the direction of roads and the location of any shop and crossroads. 

In contrast to refreshable braille displays, tablet/smartphone-integrated haptic actuators may not be able to provide guidance cues because the vibrators can vibrate only along one axis. 
However, it can supplement map applications installed on tablets or smartphones. 
For example, they actuate when the users' finger moves on the road so that they will know where they should make a turn or cross the road. 

Aside from tablet/smartphone-integrated haptic actuators, haptic mice should be used with computers and thus are unsuitable for outdoor use. 
Additionally, haptic gloves have been demonstrated to provide continuous guidance cues to BLV users by creating directional skin-stretch on the backside of the hands \cite{chase2020pantoguide}. 
Therefore, researchers can also explore how haptic gloves can assist BLV users' guidance/navigation. 

% In comparison, haptic sliders and robotic-arm haptic devices are commonly grounded and thus cannot be used for guidance/navigation. 
3D models are non-refreshable, making them unable to provide continuous guidance cues and detect obstacles, and thus are not suitable for guidance/navigation tasks. 
In summary, with further development, refreshable braille displays/pin arrays and haptic gloves hold promise for assisting BLV people in guidance/navigation, while tablet/smartphone integrated haptic actuators may supplement the use of map applications.

\subsubsection{Underexplored haptic tools for education/training}
Haptic sliders and haptic bands were not used for education/training. 
% The potential reason is that their form factors are rarely used to convey graphical information, which is a key part of STEM education (e.g., math, physics, biology, and chemistry) and O\&M training \cite{melfi2020understanding,petit2008refreshable}.
In this context, haptic devices should allow the teachers to edit their lecture materials easily because they typically must make repeated revisions before teaching \cite{melfi2020understanding}. 
Haptic sliders, with certain modifications, may be able to assist BLV users in graphical information understanding, and further assist BLV students in learning graphs and charts during class because the graphs are important in STEM education and O\&M training. 
For example, they can learn the trend of charts in math class and the map in O\&M class by moving the sliders to each location and memorizing their different sensations (e.g., different finger inclinations), which has been achieved by prior works \cite{fan2022slide,gay2021f2t}. 

% Compared to haptic sliders, haptic bands would only be capable of assisting with education/training if they can be worn on the finger and convey graphical information, which we mentioned in the second paragraph of section \ref{Haptic Assistive Tools for Understudied Application areas}. 
Compared to haptic sliders, haptic bands would be more easily applied to education/training if they could be worn on the finger and convey graphical information.
Haptic bands need to incorporate additional improvements such as reduced noise production and risk of interruption. They should also be light because the students have to use them for a prolonged period during class. 
\rv{For BLV people, fingers are vital for perceiving the environment in daily life. Therefore, future researchers developing wearable haptic bands must carefully address how to avoid interfering with the natural functions of the fingers. 
For instance, they could adopt unobtrusive design approaches for the form factor, as demonstrated in previous works \cite{jiang2024designing, tanaka2023full}.}

% In comparison, white canes have been widely used for O\&M training, though we found no papers from our literature review. The reason may be that the white canes have been used for O\&M training for a long time and are a traditional and classical method, so researchers currently focus on applying white canes to other tasks like guidance/navigation.

\subsection{Haptic Feedback for Various Tasks} \label{Haptic Feedback for Various Tasks}
In addition to describing the types of haptic assistive tools that support the main tasks, we also categorized the types of haptic feedback used for various tasks. These include \textbf{pressure} (79/132), \textbf{kinesthetic feedback} (36/132), \textbf{vibration} (32/132), \textbf{skin-stretch} (9/132), and \textbf{thermal feedback} (1/132), as shown in Table \ref{table:type_of_haptic_feedback}. \textbf{Pressure} is produced by applying a normal force to the stimulation area, such as using raised lines and dots from tactile graphics/maps \cite{wang2020multimodal}, shown in Figure \ref{fig:task_haptic_feedback} a.1). \textbf{kinesthetic feedback} is induced by a multi-degree-of-freedom force and torque feeling related to the awareness of the position or the shape of grasped objects, such as by pulling with drones, robots, and robotic arms\cite{purves2019neurosciences}, shown in Figure \ref{fig:task_haptic_feedback} b.1). \textbf{Vibration} is induced by the vibration of actuators, such as voice coil actuators, linear resonant actuators, and piezo-electric actuators \cite{lim2021systematic}, shown in Figure \ref{fig:task_haptic_feedback} c.1). \textbf{Skin-stretch} is induced by applying tangential force to the stimulation area, such as by the motors' rotation \cite{wang2020multimodal}, shown in Figure \ref{fig:task_haptic_feedback} d.1). \textbf{Thermal feedback} is induced by temperature stimulation to thermoreceptors, such as by Peltiers, which is a thermal control module that has both "warming" and "cooling" effects and can quickly change the temperature \cite{nasser2020thermalcane}, and thermal liquid. They respond over a temperature range of 5 °C–45 °C, and a sharp temperature change can cause pain \cite{huang2022recent,jones2008warm}, shown in Figure \ref{fig:task_haptic_feedback} e.1). 




\begin{table}[htbh!]
\caption{Type of haptic feedback}
\centering
\renewcommand{\arraystretch}{1.5} % Adjust row height
\small % Smaller font size
\begin{tabular}{p{2.5cm}p{3cm}p{2cm}p{3cm}p{3cm}}
\hline
\textbf{Type of Haptic Feedback} & \textbf{Graphical Information Understanding} & \textbf{Guidance /    
  Navigation} & \textbf{Education/ Training} & \textbf{Other Life and Work Tasks} \\
\hline
Kinesthetic feedback & \cite{soviak2016tactile,guinness2019robo,ducasse2016tangible,abu_doush2009making,abu2010multimodal,moll2013haptic,ducasse2018botmap,de_felice2007haptic,sallnas2007group,schloerb2010blindaid,gay2021f2t,park2015telerobotic} & \cite{siu2020virtual,huppert2021guidecopter,swaminathan2021from,guerreiro2019cabot,nasser2020thermalcane,kayukawa2020guiding,zhao2018enabling,amemiya2009haptic,amemiya2010orienting,rahman2023take,moon2019prediction,tanabe2021identification,wang2012halo,kim2015identification} & \cite{zhang2017multimodal,espinosa2021virtual,crossan2008multimodal,plimmer2011signing,murphy2015haptics} & \cite{das2023simphony,lieb2020haptic,Morelli2010vi,Plimmer2008multimodal,Park2013real} \\
\hline
Vibration & \cite{yatani2012spacesense,palani2017principles,quek2013enabling,sharmin2005first,yoo2022perception,chu2022comparative,jiang2024designing} & \cite{siu2020virtual,hong2017evaluating,erp2020tactile,Kaul2021around,kayukawa2020guiding,hirano2019synchronized,cosgun2014evaluation,lee2023novel,flores2015vibrotactile,zhao2018enabling,xu2020virtual,wang2012halo,kim2015identification,ogrinc2018sensory} & \cite{Toennies2011toward,oliveira2012the} & \cite{fink2023autonomous,sucu2014the,Stearns2016evaluating,Allman2009rock,Morelli2010vi,Cassidy2013haptic,Headley2011roughness,Rantala2009methods,Strachan2013vipong} \\
\hline
Skin-stretch & \cite{fan2022slide,kim2011handscope,gay2021f2t,chase2020pantoguide} & \cite{liu2021tactile,spiers2017design} & \cite{sanchez2010usability} & \cite{Tanaka2016haptic,kayhan2022a} \\
\hline
Thermal feedback & / & \cite{nasser2020thermalcane} & / & / \\
\hline
Pressure & \cite{shi2016tickers,swaminathan2016linespace,li2019editing,yang2020tactile,reinders2020hey,brule2021beyond,hofmann2022maptimizer,holloway20223D,fan2022slide,holloway2023tacticons,Nagassa20233D,baker2014tactile,lucentmaps2016gotzelmann,reichinger2016gesture,shi2017designing,suzuki2017fluxmarker,guinness2019robo,baker2016tactile,visually2018gotzelmann,reichinger2018pictures,prescher2017consistency,gupta2019evaluating,zeinullin2022tactile,brayda2015the,besse2018understanding,kim2015toward,braier2014haptic,mcGookin2010clutching,kim2011handscope,prescher2010tactile,kane2013touchplates,wang2009instant,ducasse2016tangible,shi2019designing,rao20202across,ducasse2018botmap,quek2013enabling,roberts2005haptic,sharmin2005first,Deschamps2012interpersonal,mascle2022tactile,levesque2012adaptive,pietrzak2009creating} & \cite{huppert2021guidecopter,barontini2021integrating,rahman2023take,spiers2017design} & \cite{albouys2018towards,holloway2018accessible,melfi2020understanding,davis2020tangible,chang2021accessiblecircuits,fusco2015tactile,holloway20193d,saikot2022refreshable,sanchez2010usability,petit2008refreshable,sargsyan20233D,oliveira2012the,brayda2013predicting,melfi2022audio} & \cite{Guo2017facade,bornschein2018comparing,Jung2021ThroughHand,das2023simphony,fink2023autonomous,bornschein2015collaborative,siu2019shapecad,baldwin2017the,Morash2018evaluating,Siu2019Advancing,Cassidy2013haptic,shi2020molder,pandey2020explore,lee2023tacnote,Headley2011roughness,Pantera2021lotusbraille} \\
\hline
\end{tabular}
\label{table:type_of_haptic_feedback}
\end{table}


\begin{figure} [tbh!]
    \centering
    \includegraphics[scale=0.23]{figure/task_haptic_feedback.jpg}
     \caption{Examples of haptic feedback mechanisms and usage in various papers. The overlaps show a combination of various haptic feedback.}
     \Description{This figure illustrates the mechanisms of 5 haptic feedback and their relationships. The numbers represent the number of papers utilized based on the haptic feedback.}
    \label{fig:task_haptic_feedback}
\end{figure}

  

\subsubsection{Haptic feedback for graphical information understanding}
\textbf{Pressure} is the most used type of haptic feedback in assisting graphical information understanding (43/58), followed by \textbf{kinesthetic feedback} (12/58), \textbf{vibration} (7/58), and \textbf{skin-stretch} (4/58). \textbf{Pressure} is induced by the BLV user's touch and stroke on the raised lines and dots. The users memorize the location and shape of the lines and the combination and arrangement of a series of dots to build the images' overview gradually \cite{yang2020tactile,melfi2020understanding,shi2019designing,soviak2016tactile,brayda2015the,fan2022slide,guinness2019robo,yatani2012spacesense}. 

\textbf{Vibration} rendered graphical information by vibrating when the user's fingers touched the lines of graphs presented on the smartphone or tablet's screen. The BLV users build an overview of the graphs by continuously feeling and memorizing the locations and connections of the lines. These vibrators could either be integrated with the mobile device \cite{Toennies2011toward} shown in Figure \ref{fig:tablet_smartphone_integrated_haptic_actuators} c), or attached to an environmental device \cite{yatani2012spacesense,sharmin2005first}.

\begin{figure} [tbh!]
    \centering
    \includegraphics[scale = 0.8]{figure/tablet_smartphone_integrated_haptic_actuators.jpg}
     \caption{Examples of tablet smartphone integrated haptic actuators: a) a tablet/smartphone integrated haptic actuator system that assists BLV people interacting with touchscreens with based on vibration \cite{chu2022comparative}; b) A tablet/smartphone haptic device that conveys graphical and mathematical concepts through vibration and audio cues \cite{Toennies2011toward}.}    
     \Description{This figure illustrates the examples of tablet smartphone integrated haptic actuators, each figure includes three subfigures. Each subfigure shows one prototype.}
     \label{fig:tablet_smartphone_integrated_haptic_actuators}
\end{figure}

\subsubsection{Haptic feedback for guidance/navigation}
\textbf{Kinesthetic feedback} (14/26) and \textbf{vibration} (14/26) are the most used haptic feedback in assisting guidance/navigation, followed by \textbf{pressure} (4/26), \textbf{skin-stretch} (2/26), and \textbf{thermal feedback} (1/26). Robots and drones leveraged \textbf{kinesthetic feedback}  \cite{huppert2021guidecopter} or integrated with other feedback to guide BLV users when they walk along a predefined trajectory  \cite{nasser2020thermalcane}. 

\textbf{Pressure} was integrated with \textbf{skin-stretch} and \textbf{kinesthetic feedback} to provide haptic direction cues to guide users when walking \cite{barontini2021integrating,spiers2017design}. \textbf{Thermal feedback} assists BLV people's guidance by changing the temperature and application direction to indicate go or stop and help them find their way  \cite{nasser2020thermalcane}.

\subsubsection{Haptic feedback for education/training}
\textbf{Pressure} (14/20) and \textbf{kinesthetic feedback} (5/20) are the most used haptic feedback in supporting education/training, followed by \textbf{vibration} (2/20) and \textbf{skin-stretch} (1/20). \textbf{Pressure} mainly assists the education of graphical-related knowledge, such as geometry\cite{petit2008refreshable,melfi2022audio} and geography \cite{albouys2018towards,holloway20193d,holloway2018accessible}. One study used the combination of pressure and skin-stretch to improve BLV students' navigation skills \cite{sanchez2010usability}. Robotic arms leverage \textbf{kinesthetic feedback}  to guide BLV users' fingers to provide an intuitive understanding of charts and 2D shapes in math education\cite{abu2010multimodal,espinosa2021virtual}, biology \cite{murphy2015haptics}, and children's handwriting \cite{plimmer2011signing}. 

\textbf{Vibration.} When BLV users touched lines and shapes on the touchscreens, a vibration was applied to help them recognize shapes \cite{Toennies2011toward,palani2017principles}. In addition, \textbf{vibration} was integrated with pressure to assist BLV students with focusing on the whiteboard the instructor is pointing at, thus bringing them back to mainstream classrooms \cite{oliveira2012the}. 

\subsubsection{Haptic feedback for other life and work tasks}
\textbf{Pressure} (16/28) and \textbf{vibration} (9/28) are the most used haptic feedback in assisting other life and work tasks, followed by \textbf{kinesthetic feedback} (3/28) and \textbf{skin-stretch} (2/28). \textbf{Pressure} is applied to assist BLV users with hand drawing/writing \cite{bornschein2018comparing,pandey2020explore}, interacting with appliances \cite{Guo2017facade,baldwin2017the}, gaming \cite{Jung2021ThroughHand}, weaving \cite{das2023simphony}, driving \cite{fink2023autonomous}, assistive tool design \cite{bornschein2015collaborative,shi2020molder}, 3D modeling \cite{siu2019shapecad}, braille reading \cite{Morash2018evaluating,Pantera2021lotusbraille}, annotation \cite{lee2023tacnote}, and roughness perception \cite{Headley2011roughness}. 

\textbf{Vibration} was leveraged by vibrators to provide direction cues in assisting BLV drivers \cite{sucu2014the} and improve the game experience \cite{Strachan2013vipong,Morelli2010vi,Allman2009rock}. \textbf{kinesthetic feedback} was provided by robotic arms' guidance to assist BLV people with 3D modeling \cite{lieb2020haptic}, hand drawing/writing, and telepresence \cite{Park2013real}. \textbf{Skin-stretch} is induced by BLV people moving the haptic slider for audio production \cite{Tanaka2016haptic}.

\subsection{Exploring Haptic Feedback: Usage, Comparisons, and Future Applications - Discussion for Haptic Feedback for Various Tasks}
Our findings demonstrated how five types of haptic feedback were used for different tasks, and we further discuss each haptic feedback in this section. 
We first describe the utilization of various haptic feedback in different tasks, including graphical information understanding, guidance/notification, education/training, and other tasks (e.g., cooking and baking). We then make comparisons with other haptic feedback to explain their respective strengths and limitations. 
Finally, we discuss the potential applications of each haptic feedback for future research.

\subsubsection{Potential usage of kinesthetic feedback}
Kinesthetic feedback is induced when mechanoreceptors within the joints and muscles detect the body's movement or halt due to force applied by actuators. 
Our literature review showed that kinesthetic feedback has been widely used for all tasks. 
BLV people utilize kinesthetic feedback to perceive the movement of their arms, aiding in understanding the contours of 2D graphs, shapes of 3D models, and directional cues provided by robotic-arm haptic devices and robot/drone haptic devices \cite{lieb2020haptic,zhang2017multimodal,espinosa2021virtual,huppert2021guidecopter,guinness2019robo}. 
Alternatively, they sense abrupt halts in hand movement caused by force applied to the hands, aiding in obstacle detection while using white canes \cite{nasser2020thermalcane,xu2020virtual,swaminathan2021from}.
Compared to pressure and skin-stretch, kinesthetic feedback necessitates precise force application to either facilitate or impede body movement \cite{park2020effect}. 
Therefore, while kinesthetic feedback can offer clear haptic cues due to its effective force, it requires more powerful actuators that are typically larger and heavier \cite{see2022touch}.
% Despite these drawbacks, in principle, kinesthetic feedback can be employed in any task benefiting from haptic guidance cues and notifications. 
Despite these drawbacks, kinesthetic feedback may be employed in tasks that involve haptic guidance cues and notifications.
For instance, in education/training, it can assist BLV users in painting or sculpting by guiding their hands along painting or cutting trajectories. 
In baking, it can facilitate ingredient search and addition step by step. 

\subsubsection{Potential usage of vibration}
Vibration occurs when mechanoreceptors under the skin detect the vibrating actuators. 
Our literature review indicates widespread use of vibration across tasks, except for education/training. 
BLV people perceive guidance cues generated by haptic bands' vibrations for navigation or gaming \cite{hong2017evaluating,erp2020tactile,flores2015vibrotactile}, or they sense notifications while touching lines and graphs on smartphones \cite{yoo2022perception,chu2022comparative}. 
Unlike other haptic feedback methods, vibration is cost-effective, requiring lower power consumption, and its low-profile vibrators can be discreetly attached under clothing or surfaces.
However, it may not offer as precise haptic cues as kinesthetic feedback \cite{ooka2010virtual}. 
Vibrators attached in different locations produce varying direction cues, with closer placements providing higher resolution. 
Yet, kinesthetic feedback, utilizing motor rotation, offers substantially higher resolution, around 0.18 degrees, surpassing vibration \cite{kaneko1989spherical}.
Nevertheless, despite its limitation in rendering high-resolution haptic guidance cues, vibration still finds utility in education/training. 
For instance, it can simulate object weight to aid BLV children in understanding weight differences. 
This simulation is achieved through vibrotactile phantom sensation (VPS), precisely controlling vibration magnitude and vibrator location. 
Maintaining constant magnitude while adjusting vibrator distance generates tangential force while maintaining magnitude and moving vibrators back and forth generates slip \cite{ooka2010virtual}.  

\subsubsection{Potential usage of skin-stretch}
Skin-stretch arises when sheer force activates mechanoreceptors. 
Our literature review uncovered fewer than five instances where skin-stretch was employed across all four tasks. 
BLV users either perceived skin-stretch through the movement of haptic sliders to grasp graphic contours \cite{fan2022slide,kim2011handscope}, or they sensed it from motors' rotation, providing continuous guidance cues \cite{liu2021tactile,spiers2017design}. 
Both tasks rely on haptic guidance cues provided by skin-stretch, although its effectiveness is somewhat limited without the ability to vary haptic intensities, unlike other types of feedback.
However, skin-stretch offers guidance with compact, lightweight mechanical structures, typically employing just a servo motor, making it portable. 
We found that skin-stretch devices are suitable for on-the-go guidance/navigation, supported by an example from Liu et al. \cite{liu2021tactile}.
Skin-stretch devices excel in indoor O\&M training due to their compactness and lightness.
\rv{When combined with vibration, skin-stretch devices can offer both haptic guidance and notifications mirroring real BLV usage scenarios.
For example}

% Unlike traditional training tools like white canes, which only detect barriers, skin-stretch devices, when combined with vibration, offer haptic guidance and notifications mirroring real BLV usage scenarios (e.g., using white canes alongside smartphone guidance).

\subsubsection{Potential usage of thermal feedback}
Thermal feedback occurs when temperature changes activate thermal receptors. 
Our investigation uncovered only one instance of thermal feedback used in guidance/navigation, with no instances in the other tasks.
BLV people perceive guidance cues through thermal feedback stimulation from peltiers. 
Unlike other haptic feedback types, thermal feedback is susceptible to environmental temperature and clothing effects \cite{halvey2011effect,halvey2012baby}.  
However, it offers versatility in conveying both haptic guidance and notification cues across various applications.
In cooking and baking, it may provide food temperature information, offering a more intuitive experience and protecting BLV individuals from burns compared to audio notifications, which was discussed in Section \ref{Haptic Assistive Tools for Understudied Application areas}.
For graphical information understanding, wearing peltiers on fingertips can signify different map areas through temperature changes. 
For example, when they touch buildings, the temperature rises to represent the indoor environment, and when they touch the street or other outdoor locations, the temperature falls to represent the outdoor environment. 
For education/training, thermal feedback may aid with understanding objects or creatures. 
For instance, a temperature drop could indicate cold-blooded animals like snakes, while a rise could suggest warm-blooded ones like rabbits.

\subsubsection{Potential usage of pressure}
Pressure feedback is generated when normal force stimulates mechanoreceptors.
We found fewer than five instances of pressure used in guidance/navigation.
BLV users commonly perceive height variations across graphs through tactile graphics/maps, refreshable braille displays/pin arrays, haptic mice, and gloves \cite{swaminathan2016linespace,Jung2021ThroughHand,Nagassa20233D,siu2019shapecad,prescher2017consistency}, or sense shapes of 3D models, robot/drone haptic devices, handheld devices, and haptic sliders \cite{shi2016tickers,huppert2021guidecopter,fan2022slide,brayda2015the,goncu2010usability}. 
% Pressure is the most widely used haptic feedback among all types.
% Unlike other haptic devices, pressure devices can be as simple as tactile maps or 3D models, making them lightweight and easy to create, hence their widespread use. 
% However, pressure is less utilized than kinesthetic feedback and vibration for guidance/navigation. 
% This is partly due to larger, heavier pressure guidance devices compared to vibration-based ones and lower guidance accuracy (0.18 degrees, achieved by motor rotation) compared to kinesthetic feedback. 

% Therefore, pressure is better suited for other tasks. 

Pressure is one of the most commonly used forms of haptic feedback. 
Unlike many other haptic technologies, pressure-based devices can range from simple tactile maps to 3D models, which makes them relatively lightweight and easy to produce, contributing to their broader application. 
However, pressure was used less frequently than kinesthetic feedback and vibration for guidance and navigation purposes. 
This is partly because pressure-based guidance devices tend to be larger and heavier compared to vibration-based alternatives, and they offer lower guidance accuracy (0.18 degrees, achieved through motor rotation) in comparison to kinesthetic feedback. 
As a result, pressure may be applied to other types of tasks that simulate the perception of holding objects.
For instance, haptic gloves can simulate holding virtual chess or laser guns, enabling BLV people to play chess and First-Person Shooter (FPS) games without visual cues \cite{qi2023haptglove}.   
By mimicking the sensation of holding chess pieces or laser guns, BLV players can engage in virtual gaming with spatial awareness cues provided by sound direction and intensity changes.





\subsection{On-body Stimulation Position for Tasks} \label{Stimulation Position for Tasks}
Haptic assistive tools produced haptic feedback on eight on-body stimulation positions, which include \textbf{finger} (101/132), \textbf{hand} (37/132), \textbf{wrist} (5/132), \textbf{waist} (4/132), \textbf{ankle} (2/132), \textbf{arm} (2/132), \textbf{shoulder} (1/132), \textbf{foot} (1/132), and \textbf{head} (1/132). Figure \ref{fig:stimulation_position} shows the distribution of BLV people's tasks in each on-body stimulation position. 


\begin{figure} [tbh!]
    \centering
    \includegraphics[scale=0.65]{figure/Stimulation_position.png}
     \caption{BLV tasks achieved by stimulating different on-body stimulation positions: the bars illustrate the frequency of each on-body stimulation position utilized for different tasks.}
     \Description{This figure illustrates the on-body stimulation positions pointed to a human's body figure. The on-body stimulation positions include finger, hand, wrist, waist, ankle, arm, shoulder, foot, and head. The bars near each on-body stimulation position illustrate the frequency of each on-body stimulation position utilized for different tasks.} 
     \label{fig:stimulation_position}
\end{figure}

\subsubsection{Finger} 
The \textbf{finger} is most used for graphical information understanding (55/101), followed by other life and work tasks (24/101) and education/training (18/101), and is least used for guidance/navigation (4/101). 

BLV users used their \textbf{finger} to touch and stroke the raised lines, dots, and shapes of the tactile graphics/maps, refreshable braille displays/pin arrays, and 3D models. The pressure induced by touching and stroking helped them build an overview of the graphical information and continuously update this overview \cite{shi2016tickers,petit2008refreshable}. BLV users could also sense vibrations when touching images on the smartphone's touchscreen and gradually explored the border and shape of the images \cite{palani2017principles,yoo2022perception}. 
Other haptic feedback induced on the \textbf{finger} include skin-stretch from a slider and mouse \cite{fan2022slide,kim2011handscope,gay2021f2t} and kinesthetic feedback from robotic arms to guide their \textbf{finger} along the predefined trajectory of images, which assisted BLV users in understanding their content \cite{park2015telerobotic,schloerb2010blindaid}.

For other life and work tasks, the \textbf{finger} perceived the relative height changes of refreshable braille displays/pin arrays' actuators or pins to build the 3D models and to read braille characters \cite{Guo2017facade,Siu2019Advancing,Morash2018evaluating}. 
The \textbf{finger} could also perceive the vibration from actuators attached to a haptic band or haptic mouse to generate roughness sensations in graphs or to indicate the impact of a ball in a haptic game \cite{Stearns2016evaluating,Headley2011roughness,Strachan2013vipong}. 
Furthermore, the kinesthetic feedback from the robotic arms guided the \textbf{finger} along a predefined trajectory \cite{Plimmer2008multimodal,Park2013real}. 

To assist with education/training, \textbf{finger} perceived pressure from various 3D models to distinguish the map's features for O\&M training and the structure of a circuit board based on differences in shapes \cite{chang2021accessiblecircuits,fusco2015tactile}, and kinesthetic feedback from robotic arms to help students explore the 3D shapes in class and learn handwriting \cite{espinosa2021virtual,plimmer2011signing}. 

To assist guidance/navigation, \textbf{finger} perceived pressure and skin-stretch from the pull of drones and robots \cite{huppert2021guidecopter,rahman2023take} shown in Figure \ref{fig:robot_drone_haptic_devices} a) and b), and the deformation of other handheld haptic devices \cite{liu2021tactile, spiers2017design}, shown in Figure \ref{fig:other_handheld_haptic_devices} a) and Figure \ref{fig:other_handheld_haptic_devices} b). 


\subsubsection{Hand} 
The \textbf{hand} is the most used for guidance/navigation (14/37), graphical information understanding (13/37), other life and work tasks (9/37), and education/training (1/37). Compared to the \textbf{finger} that can sense finer haptic cues such as pressure and skin-stretch by touching and stroking in a small area, the \textbf{hand} has a larger contact area with the haptic assistive tools on its palmer and backside. 

Haptic assistive tools mainly applied kinesthetic feedback on the \textbf{hand} to assist with guidance/navigation, where the \textbf{hand} perceived kinesthetic feedback by holding a white cane to sense the obstacles on the road \cite{nasser2020thermalcane,zhao2018enabling} and by following the guidance of the robots and drones via holding their handles, to walk along the streets \cite{rahman2023take,guerreiro2019cabot}. 

To assist with graphical information understanding, the hands' palmer side was used as a supplement to fingers to strengthen the sensation of lines and shapes \cite{reinders2020hey,brule2021beyond}. The \textbf{hand} also sensed the vibration from a series of vibrators attached to the back of the smartphone that were distributed in a matrix shape. Each vibrator represented one place on the map and the users could understand the spatial relationships between these places by sensing the difference of vibrating locations \cite{yatani2012spacesense}.

To assist with other life and work tasks, haptic assistive tools also applied pressure and vibration on the whole \textbf{hand}, such as the pressure from a mid-air haptic device that presented the map of a street intersection by applying different pressure on the palm \cite{fink2023autonomous}
Another example includes pressure from a pin array system in a tactile game. The game required the players to sense moles and hit them with finger presses. The sensation of moles was created by pressure because of the pins' rise \cite{Jung2021ThroughHand}.

\begin{figure} [tbh!]
    \centering
    \includegraphics[scale = 0.8]{figure/other_handheld_haptic_devices.jpg}
     \caption{Examples of other handheld haptic devices: a) Tactile Compass: a holdable haptic device that guides BLV people to travel independently based on the skin-stretch guidance cues \cite{liu2021tactile}; b) A shape-changing haptic device that conveys direction cues for BLV people's navigation \cite{spiers2017design}; c) VI-Bowling: a holdable haptic device for BLV people's gaming. The figure shows how BLV users leverage the device to play Blind Hero and VI Tennis (two games) \cite{Morelli2010vi}.}
     \Description{This figure illustrates the examples of other handheld haptic devices, each figure includes three subfigures. Each subfigure shows one prototype.}
    \label{fig:other_handheld_haptic_devices}
\end{figure}

\begin{figure} [tbh!]
    \centering
    \includegraphics[scale = 0.8]{figure/robot_drone_haptic_devices.jpg}
     \caption{Examples of robot/drone haptic devices: a) GuideCopter: a drone-based haptic guidance interface to assist BLV users in finding objects \cite{huppert2021guidecopter}; b) A guiding system based on tablet robots to assist BLV people in finding objects on the table \cite{rahman2023take}; c) A guiding system that assists BLV people to walk in public spaces and to avoid pedestrians \cite{kayukawa2020guiding}.}
     \Description{This figure illustrates the examples of robot/drone haptic devices, each figure includes three subfigures. Each subfigure shows one prototype.}
    \label{fig:robot_drone_haptic_devices}
\end{figure}

\subsubsection{The other on-body stimulation positions} The other on-body stimulation positions were used in fewer than or equal to five tasks. 
The \textbf{wrist} was used to assist with guidance/navigation (4/5) and other life and work tasks (1/5), specifically during gaming via vibration from the vibrators attached to the haptic bands \cite{Allman2009rock,grussenmeyer2017evaluating,lee2023novel,siu2020virtual,ogrinc2018sensory}. The \textbf{waist} was used to assist guidance/navigation (3/5) and other life and work tasks (1/5) with haptic bands attached to the \textbf{waist}, like in the form of a belt.
The vibrators were uniformly attached to the haptic bands in an equal adjacent distance. 
The direction cues were provided by vibrating the vibrators in the appropriate direction \cite{erp2020tactile,cosgun2014evaluation,flores2015vibrotactile,kayhan2022a}. 
Specifically, one work applied this technique to assist BLV runners during their running process \cite{kayhan2022a}. 
The \textbf{arm} was used to assist guidance/navigation (1/2) and other life and work tasks (1/2), specifically during gaming via pressure, skin-stretch, and vibration induced by vibrators and motors from haptic bands \cite{barontini2021integrating,Allman2009rock}.
The haptic bands worn on the \textbf{arm} were all on the upper \textbf{arm}, which was a different location than the haptic bands worn on the wrist. 
In particular, one paper leveraged both \textbf{arm} and wrist to convey vibration cues to indicate targets to be hit in a game. 
The vibration of the \textbf{arm} indicated the farther target, while the vibration of the wrist indicated the nearer target \cite{Allman2009rock}. 
The \textbf{ankle} (2/2) and the \textbf{shoulder} (1/1) were used to assist guidance/navigation via vibration induced by haptic bands\cite{hirano2019synchronized,xu2020virtual}.
Xu et al. asked the BLV participants to wear a backpack that was attached to four vibrators in three arrangements. 
All the arrangements included the attachment of two fixed vibrators on the \textbf{waist}, while the other two vibrators were attached to the \textbf{shoulder}, the \textbf{ankle}, and the \textbf{wrist} individually. 
The fixed two vibrators indicated left and right direction while the other two vibrators on the \textbf{waist} indicated go and stop. 
They compared the guiding performance of these three arrangements and found that attaching the other two vibrators on the \textbf{shoulder} could present the highest guidance accuracy \cite{xu2020virtual}. 
The \textbf{foot} (1/1) was used to assist with education. 
Sanchez et al. developed a grounded haptic assistive tool that assist blind children in learning navigation skills by sensing the pressure and skin-stretch from the device that indicated the direction cues \cite{sanchez2010usability}. 
The \textbf{head} (1/1) assisted BLV people's navigation by using 24 vibrators around the \textbf{head}. 
The device could notify the users to move and stop and provide direction cues by vibrating different groups of vibrators. 
They found that, their device could achieve an average absolute deviation of 5.7 cm  from the predefined trajectories \cite{Kaul2021around}. 

\subsection{Rarely-used On-body Stimulation Positions for Various Tasks - Discussion for On-body Stimulation Position for Tasks} \label{Rarely-used Stimulation Positions For Various Tasks}
The results of how on-body stimulation positions are used for different tasks showed that certain on-body stimulation positions are rarely used in applications.
Specifically, our findings indicate that the finger and hand are the most commonly employed on-body stimulation positions, whereas the wrist, waist, ankle, arm, shoulder, foot, and head are utilized in only five instances or less.
In the subsequent discussion, we explore the potential factors contributing to this pattern and suggest possible avenues for future research.

\subsubsection{Two-point Discrimination of Various On-body Stimulation Positions}
Previous research has utilized a metric known as successive two-point discrimination to ascertain the distribution of mechanoreceptors across different regions of the human body. 
This metric measures the minimal distance at which two stimuli can be distinguished when applied successively \cite{dellon1987reliability}. 
A lower two-point discrimination value indicates a higher density of mechanoreceptors and increased sensitivity to position.
The finger exhibits the highest distribution of mechanoreceptors (0.3 cm), followed by the hand (0.4 cm for the palm, 0.9 cm for the dorsum), head (0.6 cm for the forehead), foot (0.6 cm for the sole, 1.4 cm for the dorsum), waist (1.2 cm for the back), arm (1.5 cm for the forearm), wrist (1.7 cm), and shoulder (1.9 cm)  \cite{koo2016two,mancini2014whole}.
Our literature review reveals that the utilization of various on-body stimulation positions in the examined papers partially aligns with the recognized distribution of mechanoreceptors across the human body. 
Specifically, the fingers and hands emerge as the most sensitive on-body stimulation positions and are consequently prevalent in various tasks.
However, despite the head and foot being more sensitive than the wrist, waist, arm, and shoulder, they are underutilized on-body stimulation positions. 
One explanation could be the ease of wearing haptic assistive tools on the wrist, waist, arm, and shoulder compared to the foot. 
Additionally, wearing such tools on the head may attract unwanted attention and may be less favored by BLV users.

\subsubsection{Potential Applications of Various On-body Stimulation Positions}
Although these areas are less frequently utilized, they present potential for further exploration. 
For instance, researchers could design haptic assistive tools to stimulate different areas under the sole to provide feedback mimicking various terrains such as deserts, snowfields, or rocky lands as mentioned by Wang et al. \cite{wang2018design}. 
Apart from the head and foot, other on-body stimulation positions such as the arm, wrist, waist, shoulder, and ankle are primarily utilized for wearing haptic bands for guidance/navigation but can be leveraged for additional tasks. 
For instance, haptic assistive tools could enhance the film-watching experience for BLV individuals by providing pressure and thermal feedback worn on these positions to mimic whole-body sensations, such as being bitten by a snake or feeling wind and fire in front of the users, as demonstrated by Delazio et al. through pneumatic devices \cite{delazio2018force}. 
This haptic feedback enriches the film-watching experience for BLV individuals by compensating for information lost due to lack of vision.  
Compared to traditional methods like audio descriptions, haptic assistive tools seamlessly integrate into the film-watching process without disrupting dialogue, sound effects, or musical scores \cite{viswanathan2011enhancing}. 
In summary, various on-body stimulation positions offer potential for diverse applications, although they are currently underexplored.


\subsection{Limitations of Haptic Assistive Tools and User Studies} \label{Limitations of Haptic Assistive Tools and User Studies}
Although haptic assistive tools have been designed to assist BLV people in their daily lives and work, they still contain many limitations. The main categories include \textit{hardware limitations}, \textit{functionality limitations}, and \textit{UX and evaluation method limitations}.
Under each category, we further divided the limitations into subcategories. 
% Figure \ref{fig:hardware_limitations}, Figure \ref{fig:functionality_limitations}, and Figure \ref{fig:user_limitations} summarizes the main categories, subcategories, and the associated limitations under each subcategory. 

\subsubsection{Hardware limitations} 
\label{Hardware limitations}
Hardware limitations include \textbf{environmental effects on sensors and actuators}, \textbf{conspicuous appearance and noise}, and \textbf{cumbersome and heavy devices}.
% which are shown in Figure \ref{fig:hardware_limitations}. 
\textbf{Environmental effects on sensors and actuators} describe how environmental effects, such as physical issues and user habits, affected the sensors' sampling quality and haptic perception. \textbf{Conspicuous appearance and noise} describe how the haptic assistive tools' conspicuous appearance provoked stress in BLV users and how the noise negatively affected the BLV users' perception of haptic cues. \textbf{Cumbersome and heavy devices} describe how haptic assistive tools' large size and heavy weight affected their daily use and caused inconvenience for BLV users. 

% \begin{figure} [tbh!]
%     \centering
%     \includegraphics[scale=0.35]{figure/Hardware_limitation.png}
%      \caption{Hardware limitations include three categories: external effects on sensors and actuators, conspicuous appearance and noise, and cumbersome and heavy devices.}
%      \Description{This figure illustrates the hardware limitations, including external effects on sensors and actuators, conspicuous appearance and noise, and cumbersome and heavy devices.}
%     \label{fig:hardware_limitations}
% \end{figure}

\textbf{Environmental effects on sensors and actuators} include \textit{inaccurate sensors and haptic perception due to physical issues} and \textit{imprecise haptic perception due to users' habits}. Physical issues are induced by the change in physical conditions related to the haptic assistive tools, such as the deformation of users' skin and the orientation of wearable devices around the arm because of long time wear. Some haptic devices leveraged optical sensors, such as RGB-D cameras, to recognize on-the-road obstacles and avoid them. However, these cameras vibrated when the users moved, which lowered the sensors' sampling quality by introducing signal noise. This issue impacted the application of haptic cues, common for haptic bands, robot/drone haptic devices, and other handheld haptic devices \cite{kayhan2022a}. In addition, physical issues also affected BLV users' haptic perception. 
For example, while a robot guided users, it used vibrations to warn them of obstacles. However, vibrations from the robot were hard to distinguish from those caused by the rough surface of the floor, leading to confusion \cite{kayukawa2020guiding}.

Additionally, the quality of sensor sampling and users' haptic perception were influenced by their habits. 
For example, when users wore haptic bands on the wrist for guidance while using a white cane, how they held the cane changed the relative angles of their hand to the ground. 
If the coordinates of the guiding system were based on the haptic bands rather than the ground, the direction cues would be based on the haptic bands' coordinates.
This discrepancy meant that the cues did not match the actual directions needed in the real-world, leading to inaccurate guidance \cite{kayhan2022a}. 
\rv{As mentioned by prior works, sensors' inaccuracy may cause safety issues, such as collision in a crowded place and falling due to inaccurate guidance to the surface with height differences \cite{thiyagarajan2022intelligent}.
As the safety issue is critic, additional precision for navigation is necessary.}


\textbf{Conspicuous appearance and noise} includes \textit{noise from actuators} and \textit{conspicuous haptic assistive tools}. Motors and vibrators produced noise during their operation, affecting users' perception of haptic cues and audio reports of multimodal assistive tools \cite{huppert2021guidecopter,Kaul2021around}. Specifically, Kaul et al. developed a head-worn haptic assistive tool for BLV people's guidance. However, the noise from the vibrators negatively affected BLV people's recognition because some vibrators were close to their ears. They reported that, after bone conduction, the noise was especially loud and possibly disruptive, distracting them from the direction cues \cite{Kaul2021around}. 

The conspicuous appearance of haptic assistive devices, such as robots/drones and other tools exceeding the size of a smartphone, negatively impacted BLV users. The use of these conspicuous tools drew unwelcome attention and discussion among nearby individuals and made BLV users feel uncomfortable, as they preferred not to be perceived differently due to their visual conditions \cite{kayhan2022a,guerreiro2019cabot}.

\textbf{Cumbersome devices} include \textit{Inconvenience of grounded and heavy devices}. Due to their large size and weight, stemming from their mechanical designs, robotic-arm haptic assistive tools and haptic sliders were typically mounted on a table or secured to the ground.
These tools limited user mobility, for example, teachers had to transport these heavy devices across classrooms, or BLV students had to relocate to the specific classroom equipped with the device. This arrangement was inconvenient for both teachers and BLV students \cite{murphy2015haptics,crossan2008multimodal}.

Furthermore, the size and weight of robots and drones made them impractical for everyday use, and they could pose safety risks, particularly in crowded or narrow spaces. For instance, Kayukawa et al. found that BLV users felt this equipment was ``too large and heavy for daily use,'' expressing concerns about the potential for collisions with other pedestrians in densely populated areas \cite{kayukawa2020guiding}.

\subsubsection{Functionality limitations}
\label{Functionality limitations}
Functionality limitations include \textbf{lack of information display control}, \textbf{lack of detailed information}, and \textbf{few presentation modalities}.
% which are shown in Figure \ref{fig:functionality_limitations}. 
The \textbf{lack of information display control} describes the drawbacks of limited control of their haptic assistive tools and limited refreshing and zooming functions on BLV people's image sensemaking process. The \textbf{lack of detailed information} describes the difficulties in presenting complex structure and geometry, and how the limited display resolution of graphical information fails to present complex images to the BLV users. \textbf{Few presentation modalities} describe how only using a single type of haptic feedback may affect haptic assistive tools' information convey performance.

% \begin{figure} [tbh!]
%     \centering
%     \includegraphics[scale=0.35]{figure/Functionality_limitation.png}
%      \caption{Functionality limitations include three categories: lack of information display control, lack of detailed information, and few presentation modalities.}
%      \Description{This figure illustrates the functionality limitations, including lack of information display control, lack of detailed information, and few presentation modalities.}
%     \label{fig:functionality_limitations}
% \end{figure}

\textbf{Lack of information display control} includes \textit{lack of user control of assistive tools} and \textit{non-refreshable and non-zoomable images}. The lack of user control of assistive tools includes the control of speed and intensity of haptic feedback. On one hand, the speed for haptic sliders and robotic-arm haptic assistive tools is usually fixed. This is to control the number of variables for the user study. However, users wish to adjust the speed as they may be unable to follow a fast-speed display and find a low-speed display tedious. On the other hand, the lack of control of haptic feedback intensity may induce unclear display and potential safety issues. People have various thresholds and endurance of specific haptic feedback \cite{jiang2021douleur,lin2022super}. Low intensity may create haptic cues that the user cannot perceive, while a high intensity may induce undesired stress and potential harm to the users, as the faster the haptic assistive tools' movement, the larger the force applied to the BLV users. 
If participants were unaccustomed to the movement speed, there was a risk that these devices could unexpectedly contact their fingers or hands. Such incidents could not only startle the users but also potentially cause injury \cite{abu2010multimodal,fan2022slide}. 

Tactile graphics and maps, typically produced in print form, cannot update or zoom in on images, making them less time and cost-effective compared to dynamic haptic assistive technologies like refreshable braille displays. 
Moreover, without the capability to zoom, BLV cannot access detailed levels of information within graphics, preventing them from focusing on specific areas of interest. Access to these details is crucial for the sense-making process of BLV users, thus the absence of such detailed insight can hinder their ability to fully grasp the content of the images \cite{swaminathan2016linespace}.

\textbf{Lack of detailed information} includes \textit{difficulty in presenting complex structures and geometry} and \textit{limited display resolution of graphical information}. Current tactile graphics/maps typically present a single layer of image, chart, or map. However, it is hard for BLV users to comprehend their complex indoor structures with several separated layers of tactile maps for buildings with more than one floor. In this case, a multistorey building structure should also be presented to assist BLV users with building an overview. Lack of such presentation may induce inefficient indoor navigation within a complex building, such as in an airport. In addition, some tactile maps did not provide different haptic cues to display various types of paths and areas, which resulted in BLV users' hardness df differentiating private areas from public areas and pedestrian streets from roads for vehicles. Lack of such differentiation may induce safety issues such as trespassing. How to make the above-mentioned differentiation with simple presentations is important because it can reduce users' short-term memory load of memorizing the maps and reduce their risks of undesired trespassing \cite{hofmann2022maptimizer}.

Some refreshable braille display/pin arrays suffered from low presentation resolutions, which decreased the presented images' details. Low presentation resolutions can only assist BLV users in building an overview of simple shapes or images. However, current STEM education requires the image presentation of complex structures, such as biology and geography, which is not achievable by some of the refreshable braille display/pin arrays. The lack of such presentation may induce misunderstanding of biological structures, such as the cells and landscapes important for biology and geography \cite{melfi2022audio}.

\textbf{Few presentation modalities} include \textit{lack of information due to single type of haptic feedback}. It is hard to convey multidimensional information for assistive tools that only provide one type of haptic feedback. For example, Espinosa et al. leveraged a robotic-arm haptic device to assist BLV students in learning the 3D models with the guidance of a robotic arm. However, the device can only present the models' 3D outlines and cannot render the models' texture only with kinesthetic feedback. This reduced the realism and immersion when BLV people touched the 3D models and thus failed to assist them in learning the textural features of various objects. \cite{espinosa2021virtual}.

\subsubsection{UX and evaluation method limitations}
\label{UX and evaluation method limitations}
UX and evaluation method limitations include \textbf{lack of user group diversity consideration}, \textbf{lack of customization}, \textbf{limitations on user study}, and \textbf{haptic device distrust}.
% , which are shown in Figure \ref{fig:user_limitations}. 
The \textbf{lack of user group diversity consideration} describes how the lack of consideration of users with various visual conditions, users who have different assistive tools usage habits, and users of various ages and education backgrounds affected the design and use of haptic assistive tools. The \textbf{lack of customization} describes how BLV people's user experience was affected because they could not customize their 3D models. \textbf{Limitations on user study} describes how the lack of comparison with other haptic devices, variability in the use of subjective rating scales, and lack of real-world experiments affected the design of haptic assistive tools and user studies. \textbf{Haptic device distrust} described that the BLV users distrusted the robots and drones because of their unfamiliarity with these haptic assistive tools.

% \begin{figure} [tbh!]
%     \centering
%     \includegraphics[scale=0.35]{figure/User_limitation.png}
%      \caption{Functionality limitations include four categories: lack of user group diversity consideration, lack of customization, limitations on user study, and haptic device distrust.}
%      \Description{This figure illustrates the UX and evaluation method limitations, including lack of user group diversity consideration, lack of customization, limitations on user study, and haptic device distrust.}
%     \label{fig:user_limitations}
% \end{figure}

\textbf{Lack of user group diversity consideration} includes \textit{lack of visual condition considerations}, \textit{lack of assistive tools usage habits consideration}, and \textit{lack of user ages and education background consideration}. Many haptic assistive tools were designed specifically for totally blind users, though there are more low-vision people in the world than totally blind people. Prior works have discussed their limitations: to make more BLV users use their haptic assistive tools, adding features such as sharp contrast colors for low-vision users is necessary \cite{lee2023tacnote,holloway2023tacticons}. Therefore, a lack of consideration of the BLV people's different visual conditions may exclude potential users from using the haptic assistive tools. 

Some handheld haptic devices interfered with existing assistive tools as they required users to hold the device with their dominant hand, which was typically used to hold white canes and manage guide dogs. 
Some current haptic assistive tools only have a guidance function, and users must hold the white canes or guide dogs with their non-dominant hand to recognize the obstacles \cite{liu2021tactile,spiers2017design}.
Adopting haptic assistive technologies required these users to modify their routine activities, invest time, and adapt to new techniques. The learning curve associated with these tools, along with the increased risk of bumping into obstacles during the adjustment phase, should be addressed. 

Users with various ages and educational backgrounds affected the design of haptic devices. Elders and children cannot use or wear a device for a long time due to their health conditions. Therefore, the weight should be considered when designing a handheld or wearable haptic assistive tool \cite{kayukawa2020guiding,holloway2023tacticons}. In addition, the tools designed for elders, children, and users with low education backgrounds should be easy to use as their learning efficiency is commonly lower than other users \cite{liu2021tactile,Morelli2010vi}.  Though not every work aims to provide a one-size-fits-all solution, broadening the user groups from adults only to minorities such as elders, children, and people with low education backgrounds allows us to gain a deeper understanding of their practical needs for the improvement of future prototypes.

\textbf{Lack of customization} includes \textit{Users' dissatisfaction with predefined 3D models}. The users were dissatisfied with the 3D models that did not consider the cultural and religious differences of users. For example, the Red Cross, Red Crescent, and Red Crystal were used in different regions around the world, which were all the emblems of the International Red Cross and Red Crescent Movement (IRRC) \cite{redcross2021}. However, designers without such knowledge overlooked these discrepancies and were unfamiliar with more regional, cultural, or religious symbols. Lack of such consideration may induce misunderstanding and even bias among the users \cite{holloway20223D}. In addition, BLV users require time to learn how to recognize predefined 3D icons. For instance, individuals from different generations are familiar with objects relevant to their own times but may not recognize items associated with other eras \cite{holloway2023tacticons}. The absence of customized 3D models can substantially strain short-term memory, forcing users to memorize new 3D models, particularly of objects they are not familiar with, such as specific map landmarks \cite{holloway20223D,holloway2023tacticons}.

\textbf{Limitations on user study} include \textit{lack of comparisons with other haptic devices}, \textit{variability in use of subjective rating scales}, and \textit{lack of real-world experiments}. A lack of comparisons with other haptic devices may prevent researchers from understanding the effectiveness of their devices with a known baseline. For example, Fan et al. compared their interactive haptic assistive tools with tactile graphics and 3D models to understand their line charts display performance. They found that their devices provided position and inclination cues that could assist BLV users in building an overview more intuitively than tactile graphics. Compared to 3D models, their devices provided a refreshable line chart display, which saves time for producing new 3D models \cite{fan2022slide}. While for the other works that did not compare their haptic assistive tools with the other tools, it is hard for us to ensure that their devices are competitive in performance, and thus are hard to follow by future researchers.

The variability in the use of rating scales among the studies presents a challenge in evaluating the overall user experience of these tools. 
For instance, van Erp et al. assessed mental effort using the NASA-TLX scale, which focuses on cognitive workload \cite{erp2020tactile}, while Albouys et al. employed the System Usability Scale (SUS) and the User Experience Questionnaire (UEQ) to gauge user satisfaction, without directly measuring workload \cite{albouys2018towards}. 
The inconsistency in evaluation metrics complicates comparisons across studies, making it difficult to draw meaningful conclusions about the comprehensive user experience.

Conducting research in real-world settings enhances the ecological validity of a study, offering insights into the practical use of haptic assistive tools by BLV users \cite{baxter2015chapter}. The absence of real-world experiments might fail to uncover the specific challenges, which results in overlooked design and usability problems. This impacts the overall effectiveness of the tools developed for BLV users \cite{hofmann2022maptimizer,melfi2020understanding}.

\textbf{Haptic device distrust} is shown by users' \textit{distrust of robots and drones due to unfamiliarity}. 
BLV users often experience distrust towards robots and drones due to their unfamiliarity with such technology, which differs substantially from the tools they use daily. For those who have never interacted with robots or drones, understanding their appearance and functionality is challenging, leading to feelings of insecurity. In particular, participants are concerned about collisions with robots or injuries from drone propellers, affecting both the users and bystanders \cite{kayukawa2020guiding,rahman2023take}. Furthermore, Huppert et al. reported that initial worries about drone safety were prevalent among participants, who required time to adjust to using them \cite{huppert2021guidecopter}. The challenge of ensuring drone safety was identified as a major limitation of their system, underscoring the need for additional research in this area.
